DDKSP: A Data-Driven Stochastic Programming Framework for Car-Sharing Relocation Problem

Car-sharing issue is a popular research field in sharing economy. In this paper, we investigate the car-sharing relocation problem (CSRP) under uncertain demands. Normally, the real customer demands follow complicating probability distribution which cannot be described by parametric approaches. In order to overcome the problem, an innovative framework called Data-Driven Kernel Stochastic Programming (DDKSP) that integrates a non-parametric approach - kernel density estimation (KDE) and a two-stage stochastic programming (SP) model is proposed. Specifically, the probability distributions are derived from historical data by KDE, which are used as the input uncertain parameters for SP. Additionally, the CSRP is formulated as a two-stage SP model. Meanwhile, a Monte Carlo method called sample average approximation (SAA) and Benders decomposition algorithm are introduced to solve the large-scale optimization model. Finally, the numerical experimental validations which are based on New York taxi trip data sets show that the proposed framework outperforms the pure parametric approaches including Gaussian, Laplace and Poisson distributions with 3.72% , 4.58% and 11% respectively in terms of overall profits.

==> acknowledge.tex <==
% use section* for acknowledgment
\section*{Acknowledgment}


The authors would like to thank...

==> biography.tex <==


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{20032518.jpg}}]{Xiaoming Li}
received the B.Eng. degree in computer science and technology
from Shenyang Aerospace University, China, in 2003,
and the M.S. degree in computer software and theory from Northeastern University, China, in 2009. He is currently pursuing
the Ph.D. degree in information systems engineering
with Concordia University, Canada.
His research interests include data-driven optimization, large-scale optimization, and machine learning
with applications on supply chain network design \& optimization, 5G network optimization, transportation management in intelligent transportation environments.
\end{IEEEbiography}

% if you will not have a photo at all:
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{wang.png}}]{Chun Wang}
(M’06) received the B.Eng. degree
from the Huazhong University of Science and Technology,
Wuhan, China, in 1990, and the M.E.Sc.
and Ph.D. degrees in computer engineering from
The University of Western Ontario, London, ON,
Canada, in 2004 and 2007, respectively.
He is currently an Associate Professor with the
Concordia Institute for Information Systems Engineering,
Concordia University, Canada. His research
interests include the interface between economic
models, operations research, and artificial intelligence.
He is actively conducting research in multiagent systems, data-driven
optimization, and economic model-based resource allocation with applications
to healthcare management, smart grid, and smart city environments.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{huang.jpg}}]{Xiao Huang}
obtained her Ph.D. degree from the Marshall School of Business at the University of Southern California (USC). She also holds an M.S. in Mathematical Finance from USC and B.E. in Electronic Engineering from Tsinghua University. She is currently an Associate Professor and the Concordia University Research Chair in Supply Chain Management in the John Molson School of Business at Concordia University. Her research interests involve competition and cooperation in supply chains, product and pricing strategies, and data-driven decision making.
\end{IEEEbiography}
